Effects of Turbulent Magnetic Fields on the Transport and Acceleration of Energetic Charged Particles: Numerical Simulations with Application to Heliospheric Physics

After introduction we focus on: the transport of charged particles, the acceleration of ions at shocks, and the acceleration of electrons at shocks. Chapter 2 studies the propagation of solar energetic particles(SEPs) in turbulent magnetic fields. Particle trajectories in turbulent magnetic fields are numerically integrated. The turbulence includes a Kolmogorov-like power spectrum containing a broad range of scales. Small-scale variations in particle intensities(dropouts) and velocity dispersions can be reproduced. The result gives a constraint on the error of onset analysis for inferring SEP informations. We find that dropouts are rarely produced using the two-component model(Matthaeus et al., 1990). The result questions the turbulence model. Chapter 3 studies the acceleration of ions. We use 3-D hybrid simulations to study the acceleration of low-energy particles at parallel shocks. We find that particles gain energy by reflection at the shock. The protons can move off field lines in 3-D electric and magnetic fields. We also use a stochastic integration method to study diffusive shock acceleration including large-scale magnetic variations. The results can explain the observations of anomalous cosmic rays by Voyager 1. Chapter 4 studies electron acceleration at a shock in a turbulent magnetic field by combining hybrid simulations and test-particle simulations. The acceleration is enhanced by including large-scale turbulence. Since electrons mainly follow field lines, the field-line braiding allows electrons interacting with shock many times. Ripples also contribute to acceleration by mirroring electrons. The process favors perpendicular shocks. We discuss the implication to SEPs by comparing the acceleration of electrons with that of protons. The intensity correlation of electrons and ions in SEPs implies perpendicular shocks play important roles in accelerating particles.

==> abbreviations.tex <==
\noindent ACE (spacecraft) - Advanced Composition Explorer

\noindent ACR  -  Anomalous Cosmic Rays

\noindent AU - Astronomical Unit

\noindent CME - Coronal Mass Ejection

\noindent DSA - Diffusive Shock Acceleration

\noindent ESP - Energetic Storm Particles

\noindent ISEE (spacecraft) - International Sun-Earth Explorer

\noindent GCR - Galactic Cosmic Rays

\noindent MHD - Magnetohydrodynamics

\noindent SDA - Shock Drift Acceleration

\noindent SEP - Solar Energetic Particles

\noindent SSA - Shock Surfing Acceleration

\noindent STEREO (spacecraft) - Solar TErrestrial RElations Observatory


==> abstract.tex <==
Turbulent magnetic fields are ubiquitous in space physics and astrophysics. The influence of magnetic turbulence on the motions of charged particles contains the essential physics of the transport and acceleration of energetic charged particles in the heliosphere, which is to be explored in this thesis.
After a brief introduction on the energetic charged particles and magnetic fields in the heliosphere,
the rest of this dissertation focuses on three specific topics: $1$. the transport of energetic charged particles
in the inner heliosphere, $2$. the acceleration of ions at collisionless shocks, and $3$. the acceleration of 
electrons at collisionless shocks. We utilize various numerical techniques to study these topics. In Chapter $2$ we study the propagation of charged particles in turbulent magnetic fields similar to the propagation of solar energetic particles in the inner heliosphere. The trajectories of energetic charged particles in the turbulent magnetic field are numerically integrated. The turbulence model includes a Kolmogorov-like magnetic field power spectrum containing a broad range of scales from those that lead to large-scale field-line random walk to small scales leading to resonant pitch-angle scattering of energetic particles. We show that small-scale variations in particle intensities (the so-called ``dropouts") and velocity dispersions observed by spacecraft can be reproduced using this method. Our study gives a new constraint on the error of ``onset analysis", which is a technique commonly used to infer information about the initial release of energetic particles. We also find that the dropouts are rarely produced in the simulations using the so-called ``two-component'' magnetic turbulence model \citep{Matthaeus1990}. The result questions the validity of this model in studying particle transport. In the first part of Chapter $3$ we study the acceleration of ions in the existence of turbulent magnetic fields. We use $3$-D self-consistent hybrid simulations (kinetic ions and fluid electrons) to investigate the acceleration of low-energy particles (often termed as ``injection problem'') at parallel shocks. We find that the accelerated particles always gain the first amount of energy by reflection and acceleration at the shock layer. The protons can move off their original field lines in the 3-D electric and magnetic fields. The results are consistent with the acceleration mechanism found in previous 1-D and 2-D simulations. In the second part of Chapter $3$, we use a stochastic integration method to study diffusive shock acceleration in the existence of large-scale magnetic variations. We show that the 1-D steady state solution of diffusive shock acceleration can be significantly modified in this situation. The results suggest that the observations of anomalous cosmic rays by Voyager spacecraft can be explained by a 2-D shock that includes the large-scale magnetic field variations. In Chapter $4$ we study electron acceleration at a shock passing into a turbulent magnetic field by using a combination of hybrid simulations and test-particle electron simulations. We find that the acceleration of electrons is greatly enhanced by including the effect of large-scale magnetic turbulence. Since the electrons mainly follow along the magnetic lines of force, the large-scale braiding of field lines in space allows the fast-moving electrons interacting with the shock front multiple times. Ripples in the shock front occurring at various scales also contribute to the acceleration by mirroring the electrons. Our calculation shows that this process favors electron acceleration at perpendicular shocks. We discuss the application of this process in interplanetary shocks and flare termination shocks. We also discuss the implication of this study to solar energetic particles (SEPs) by comparing the acceleration of electrons with that of protons.  The intensity correlation of electrons and ions in SEP events indicates that perpendicular or quasi-perpendicular shocks play an important role in accelerating charged particles. In Chapter 5 we summarize the results of this thesis and discuss possible future work.


%350 words for a dissertation or document.  The
%word count limits apply to the regular Abstract in the thesis and
%to the separate Special Abstract.  Use the same text for both; just
%adjust the margins and heading.  The abstract should summarize your
%work.  The UMI booklet listed in the resources section of the U of
%A manual provides some writing tips.  The abstract for a dissertation
%or document may be longer than one page; word count is more important
%than page length in this section.
%
%If you are doing a paper submission, submit one copy of the special
%abstract, and two extra copies of your title page, in the box with
%the final copies of your thesis.  If you are doing an electronic
%submission, you can ignore the special abstract.


==> acknowledgements.tex <==


\noindent First of all, I would like to thank my thesis advisor, Professor Joe Giacalone, for his
exceptional guidance and continuous support in the last five years. He has been very patient and 
spent countless time in discussion with me. He always provides selfless help and allows me to work 
on the problems I am interested in. Joe is a prototype in my scientific career.

I am very grateful to all other members in my committee. I am glad to work with Professor 
Randy Jokipii and would like to thank him for his guidance, the numerous sharp comments, and superb 
suggestions about my research projects. I appreciate Dr. Jozsef Kota for all the precious advice 
and always being a knowledgeable resource for my questions. 
I would like to thank Professor Ke Chang Hiesh for his kindness and 
serving in my thesis comittee. I want to thank Professor Roger Yelle, who keeps stimulating 
me to improve my English and other skills. I am also grateful to Professor Fulvio Melia, who used to be 
in my committee and introduced me to high-energy Astrophysics (in the well-taught class Astronomy 582).

I would like to acknowledge the help from all the members in our research group,
Marcia Neugebauer, Tami Rogers,  Federico Fraschetti, Tom Schad, Eric Greenfield, Erica McEvoy, Peng Sun, Eileen Chollet, Huirong Yan, and Chunsheng Pei. I would also like to 
express my special gratitude to our administrative associate Donita Vanture. She is such a warm-hearted lady 
and helped a lot to make our work as smooth as possible. My gratitude extends to my classmates, Nikole Lewis, Lissa Ong, Tom Schad, and Devin Schrader. It was great to have you in those classes! 
I would also like to thank all other graduate students, faculty, and staff in Lunar and Planetary 
Laboratory. You made LPL such a wonderful place to work! The last five years is such a precious and enjoyable 
memory.

I would like to thank my colleagues during my visit to Los Alamos National Laboratory, Hui Li, Shengtai Li, Hao Xu, and Wei Liu. It was a great experience and I learned a lot by working with different researchers.

%Stuart Bale, Joe Borovsky, Jih Kwin (Jerry) Chao, Ben Chandran, Yao Chen, Ed Cliver, Alan Cummings, Mihir Desai, Vladimir Florinski, Lan Jian, Rick Leske, Gang Li, Tak-Chu Li, Ying Liu, Quanming Lu, Richard Mewaldt, C. K. Ng, Gene Parker, Vahe Petrosian, Edward Stone, Hui Tian, Allan Tylka, Chenlong Shen, Linghua Wang, Yuming Wang, Gary Webb, Dan Winske, Pin (Penny) Wu and Ming Zhang.

Finally, I deeply appreciate my parents, who give me the most unconditional love and freedom to pursue what I like, and my wife Ting, for her amazing love and all the happiness she brings into my life. 


==> dedication.tex <==
\begin{center}
\emph{To Ting.}
\end{center}


